AutoMind: Adaptive Knowledgeable Agent for Automated Data Science

Large Language Model (LLM) agents have shown great potential in addressing real-world data science problems. LLM-driven data science agents promise to automate the entire machine learning pipeline, yet their real-world effectiveness remains limited. Existing frameworks depend on rigid, pre-defined workflows and inflexible coding strategies; consequently, they excel only on relatively simple, classical problems and fail to capture the empirical expertise that human practitioners bring to complex, innovative tasks. In this work, we introduce AutoMind, an adaptive, knowledgeable LLM-agent framework that overcomes these deficiencies through three key advances: (1) a curated expert knowledge base that grounds the agent in domain expert knowledge, (2) an agentic knowledgeable tree search algorithm that strategically explores possible solutions, and (3) a self-adaptive coding strategy that dynamically tailors code generation to task complexity. Evaluations on two automated data science benchmarks demonstrate that AutoMind delivers superior performance versus state-of-the-art baselines. Additional analyses confirm favorable effectiveness, efficiency, and qualitative solution quality, highlighting AutoMind as an efficient and robust step toward fully automated data science. Code is at https://github.com/zjunlp/AutoMind.

==> tables/main_old.tex <==
\begin{table*}[htp]
    \centering
    \setlength{\tabcolsep}{0.7mm}
    % \resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|cc|c|cc}
\toprule[1.2pt]
\multirow{2}{*}{\textbf{Benchmarks}} & \multirow{2}{*}{\textbf{Split}} & \multirow{2}{*}{\textbf{Metric}} & \multicolumn{2}{c|}{\textbf{Prior SOTA}} & \textbf{\begin{tabular}[c]{@{}c@{}}\ours\\ w/o Knowledge\end{tabular}} & \multicolumn{2}{c}{\textbf{\ours}} \\    
&  &  & \texttt{o3-mini} & \texttt{deepseek-v3} & \texttt{deepseek-v3} & \texttt{o3-mini} & \texttt{deepseek-v3} \\ \midrule[1pt]
\multirow{8}{*}{MLE-Bench} & \multirow{2}{*}{Easy} & Beats (\%) &
52.5 {\small± 10.8} & 74.0 {\small± 2.9} & 81.8 {\small± 0.7} \sraise{7.8} & 71.8 {\small± 4.3} \sraise{19.3} & 81.2 {\small± 0.1} \sraise{7.2} \\
& & Submissions (\#) &
93.7 {\small± 0.2} & 90.7 {\small± 33.0} & 25.8 {\small± 12.4}  & 14.6 {\small± 0.2} & 18.2 {\small± 3.3} \\
& \multirow{2}{*}{Medium} & Beats (\%) & 
20.3 {\small± 3.0} & 29.0 {\small± 6.4} & 39.2 {\small± 5.3} \sraise{10.2} & 24.9 {\small± 6.1} \sraise{4.6} & 44.3 {\small± 0.4} \sraise{15.3} \\
& & Submissions (\#) &
103.5 {\small± 44.3} & 72.3 {\small± 40.8} & 15.9 {\small± 2.2} & 8.7 {\small± 1.6} & 18.1 {\small± 9.2} \\
& \multirow{2}{*}{Hard} & Beats (\%) & 
10.7 {\small± 1.2} & 18.4 {\small± 1.8} & 23.6 {\small± 6.4} \sraise{5.2} & 36.6 {\small± 9.4} \sraise{25.9} & 38.7 {\small± 14.3} \sraise{20.3} \\
& & Submissions (\#) &
102.1 {\small± 86.8} & 36.0 {\small± 7.1} & 14.1 {\small± 6.2} & 18.9 {\small± 7.2} & 6.3 {\small± 0.7} \\ 
& \multirow{2}{*}{All} & Beats (\%) &
30.0 {\small± 0.2} & 43.3 {\small± 3.0} & 52.1 {\small± 1.0} \sraise{8.8} & 45.4 {\small± 1.7} \sraise{15.4} & 56.8 {\small± 1.4} \sraise{13.5} \\
& &Submissions (\#) &
99.5 {\small± 38.2} & 70.1 {\small± 25.9} & 19.9 {\small± 2.8} & 13.4 {\small± 2.3} & 15.2 {\small± 4.7} \\ \midrule[1pt]
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Top AI\\ Competitions\end{tabular}} & \multirow{2}{*}{OAG}            & AUC ↑                               &
0.56 {\small± 0.03} & 0.52 {\small± 0.03} & 0.50 {\small± 0.00} \sdrop{0.02} & 0.55 {\small± 0.08} \sdrop{0.01} & 0.58 {\small± 0.04} \sraise{0.06}  \\
& & Submissions (\#) &
16.0 {\small± 15.6} & 14.5 {\small± 13.4} & 48.5 {\small± 41.3} & 4.5 {\small± 2.1} & 4.0 {\small± 1.4}\\
& \multirow{2}{*}{BELKA} & AP ↑ &
0.09 {\small± 0.06} & 0.33 {\small± 0.03} & 0.19 {\small± 0.03} \sdrop{0.14} & 0.44 {\small± 0.02} \sraise{0.35} &  0.39 {\small± 0.05} \sraise{0.06} \\
& & Submissions (\#) &
5.0 {\small± 4.2} & 2.0 {\small± 0.0} & 2.5 {\small± 2.1} & 9.0 {\small± 1.4} & 8.5 {\small± 0.7}\\
\bottomrule[1.2pt]
\end{tabular}
% }
    \caption{\textbf{Main results on MLE-Bench and Top AI Competitions.} \textbf{Beats (\%)} represents the percentage of human participants surpassed by the agent on the officail leaderboard and serves as the principal evaluation metric for MLE-Bench. \textbf{Submissions (\#)} reports the number of valid submissions the agent makes within a 24-hour time budget; it is provided solely as a descriptive statistic and not as an evaluative metric, as its magnitude does not directly reflect the agent’s competence. \textbf{AUC} and \textbf{AP} are the official evaluation metrics for the OAG and BELKA competitions, respectively. Performance gains relative to the baseline are denoted by \sraise{}, whereas declines are \sdrop{}.
}
    \label{tab:main}
\end{table*}

